WinTSR: A Windowed Temporal Saliency Rescaling Method for Interpreting Time Series Deep Learning Models

Interpreting complex time series forecasting models is challenging due to the temporal dependencies between time steps and the dynamic relevance of input features over time. Existing interpretation methods are limited by focusing mostly on classification tasks, evaluating using custom baseline models instead of the latest time series models, using simple synthetic datasets, and requiring training another model. We introduce a novel interpretation method, \textit{Windowed Temporal Saliency Rescaling (WinTSR)} addressing these limitations. WinTSR explicitly captures temporal dependencies among the past time steps and efficiently scales the feature importance with this time importance. We benchmark WinTSR against 10 recent interpretation techniques with 5 state-of-the-art deep-learning models of different architectures, including a time series foundation model. We use 3 real-world datasets for both time-series classification and regression. Our comprehensive analysis shows that WinTSR significantly outperforms other local interpretation methods in overall performance. Finally, we provide a novel, open-source framework to interpret the latest time series transformers and foundation models.

==> tables/related_works_2.tex <==
\begin{table*}[!htb]
    \centering
    \caption{A summary of related works on time series interpretation methods and their comparisons.}
    \small 
    % \begin{tabular}{@{} cl*{13}c @{}} \hline
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{ |l|cc|cc|cc|cc|cc|c|} \hline
        \textbf{Related Work} &  \multicolumn{2}{c}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Scope}} & \multicolumn{2}{c}{\textbf{Evaluation}} & \multicolumn{2}{c}{\textbf{Dataset}} &\multicolumn{2}{c|}{\textbf{Task}}  & \textbf{Model} \\   \cline{2-11}
        &  {Grad.} & {Pert.}  &
        {Local} & {Global} & {Quali.} & {Quant.} & {Real} & {Syn.} & {Class.} & {Regr.} & \textbf{Agnostic}
        \\ \hline
        \citet{Choi2016RETAINAI}             &   {\LARGE \textbullet}  &    &    {\LARGE \textbullet} &   &   & {\LARGE \textbullet} & {\LARGE \textbullet} &  & {\LARGE \textbullet} & & \\
        \citet{wang2017time}             &   {\LARGE \textbullet}  &    &    {\LARGE \textbullet} &   &   & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & & \\
        \citet{ismail2019accurate}               &   {\LARGE \textbullet} &   &   {\LARGE \textbullet} &  & {\LARGE \textbullet} &  & {\LARGE \textbullet} &  & {\LARGE \textbullet} & {\LARGE \textbullet} & \\
        \citet{oviedo2019fast}              &   {\LARGE \textbullet} &     & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  & \\
        \citet{wolanin2020estimating} &  {\LARGE \textbullet} &   &    {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & & {\LARGE \textbullet} &  & & {\LARGE \textbullet} & \\
        \citet{strodthoff2019detecting}              &   {\LARGE \textbullet} &   &   {\LARGE \textbullet} &  &  & & {\LARGE \textbullet} & & {\LARGE \textbullet} &  &  \\
        \citet{siddiqui2019tsviz}              &   {\LARGE \textbullet} &    &   {\LARGE \textbullet} &  {\LARGE \textbullet} & {\LARGE \textbullet} &  & {\LARGE \textbullet} & {\LARGE \textbullet}  & {\LARGE \textbullet} & {\LARGE \textbullet}  & \\
        CPHAP \cite{cho2020interpretation}              &  {\LARGE \textbullet} &    & {\LARGE \textbullet} & {\LARGE \textbullet} &  & {\LARGE \textbullet} & {\LARGE \textbullet} &  &{\LARGE \textbullet} & {\LARGE \textbullet}  & \\
        \citet{rahim2023prediction}               &   {\LARGE \textbullet}  &       & {\LARGE \textbullet} &   & {\LARGE \textbullet} &  & {\LARGE \textbullet} & & {\LARGE \textbullet} &  & \\
        TIMEX \cite{queen2024encoding}  &   & {\LARGE \textbullet}   &   {\LARGE \textbullet} &   &   & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  & \\
        \hline
        \citet{yan2023selfinterpretable}               &   {\LARGE \textbullet}  &     & {\LARGE \textbullet} &   & {\LARGE \textbullet} & {\LARGE \textbullet} & & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  {\LARGE \textbullet}\\
        \citet{xia2023explaining}                &   {\LARGE \textbullet}  &     & {\LARGE \textbullet} &   &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & & {\LARGE \textbullet} &  {\LARGE \textbullet}\\
        \citet{kashiparekh2019convtimenet}  &    & {\LARGE \textbullet}    & {\LARGE \textbullet} &   &  &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  &  {\LARGE \textbullet}\\
        \citet{tonekaboni2019explaining}                &   & {\LARGE \textbullet}    & {\LARGE \textbullet} & {\LARGE \textbullet}  &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  {\LARGE \textbullet}\\
        FIT \cite{Tonekaboni2020WhatWW}                   &    & {\LARGE \textbullet}  & {\LARGE \textbullet} &   &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  &  {\LARGE \textbullet}\\
        
        CGS Mask \cite{lu2024cgs}                &   & {\LARGE \textbullet}   &   {\LARGE \textbullet} &   &   & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  &  {\LARGE \textbullet}\\
         \hline
        % \rowcolor{gray!25}
        % WinIT \cite{leung2022temporal}                &    & {\LARGE \textbullet}     & {\LARGE \textbullet} &   &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &{\LARGE \textbullet} &  &  {\LARGE \textbullet}\\
        % \rowcolor{gray!25}
        % TSR \cite{ismail2020benchmarking}                &  {\LARGE \textbullet}     &   & {\LARGE \textbullet} &   &  & {\LARGE \textbullet} & & {\LARGE \textbullet} & {\LARGE \textbullet} &  & {\LARGE \textbullet}\\ 
        \rowcolor{gray!75}
        \textbf{Our method - WinTSR}                &    & {\LARGE \textbullet}      & {\LARGE \textbullet} &   &  & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} & {\LARGE \textbullet} &  {\LARGE \textbullet}\\ \hline
        %\cmidrule[1pt]{1-14}
    \end{tabular}
    % }
\label{tab:TS-SaliencyInterpretation}
\end{table*}

==> tables/reproducibility.tex <==
\begin{table*}[htb]
\centering
    \caption{Reproducibility checklist}
    \small
    \begin{tabular}{|p{15.5cm}|c|} \hline
         \textbf{Question} & \textbf{Answer} \\ \hline
         Includes a conceptual outline and/or pseudocode description of AI methods introduced & yes \\
         Clearly delineates statements that are opinions, hypotheses, and speculations from objective facts and results & yes \\
        Provides well-marked pedagogical references for less-familiar readers to gain the background necessary to replicate the paper & yes \\ \hline
        Does this paper make theoretical contributions? & yes \\
All assumptions and restrictions are stated clearly and formally. & yes \\
All novel claims are stated formally & yes \\
Proofs of all novel claims are included & yes \\
Proof sketches or intuitions are given for complex and/or novel results & yes \\
Appropriate citations to theoretical tools used are given & yes \\
All theoretical claims are demonstrated empirically to hold. & yes \\
All experimental code used to eliminate or disprove claims is included & yes \\ \hline
Does this paper rely on one or more datasets? & yes \\
A motivation is given for why the experiments are conducted on the selected datasets & yes \\
All novel datasets introduced in this paper are included in a data appendix & NA \\
All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes & NA \\
All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations & yes \\
All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available & partial \\
All datasets that are not publicly available are described in detail, with an explanation of why publicly available alternatives are not scientifically satisfying. & yes \\ \hline
Does this paper include computational experiments? & yes \\
Any code required for pre-processing data is included in the appendix. & yes \\
All source code required for conducting and analyzing the experiments is included in a code appendix. & yes \\
All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. & yes \\
All source code implementing new methods have comments detailing the implementation, with references to the paper & yes \\
If an algorithm depends on randomness, then the method used for setting seeds is described sufficiently to allow results replication. & yes \\
This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries. & yes \\
This paper formally describes the evaluation metrics used and explains the motivation for choosing these metrics. & yes \\
This paper states the number of algorithm runs used to compute each reported result. & yes \\
% Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
% The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. & yes \\
This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. & NA \\
        \hline
    \end{tabular}
    \label{tab:reproducibility}
\end{table*}
